Knowledge Graph Extraction from Videos

Nearly all existing techniques for automated video annotation (or captioning) describe videos using natural language sentences. However, this has several shortcomings: (i) it is very hard to then further use the generated natural language annotations in automated data processing, (ii) generating natural language annotations requires to solve the hard subtask of generating semantically precise and syntactically correct natural language sentences, which is actually unrelated to the task of video annotation, (iii) it is difficult to quantitatively measure performance, as standard metrics (e.g., accuracy and F1-score) are inapplicable, and (iv) annotations are language-specific. In this paper, we propose the new task of knowledge graph extraction from videos, i.e., producing a description in the form of a knowledge graph of the contents of a given video. Since no datasets exist for this task, we also include a method to automatically generate them, starting from datasets where videos are annotated with natural language. We then describe an initial deep-learning model for knowledge graph extraction from videos, and report results on MSVD* and MSR-VTT*, two datasets obtained from MSVD and MSR-VTT using our method.

==> text/scrap.tex <==
\subsection{Ablation Studies}
The ablation studies show that all three of the main components of our network are relevant. In the first setting, masking out the video causes performance to drop, which means that the network is not simply guessing its logical annotation based on which atoms are most common. In the second ablation setting, using a single MLP in the decoder, rather than a different MLP for each predicate, also causes performance to drop. This means that the predicate-MLPs in our networks' decoder have learned different functions depending on the semantics of the predicate they are modelling. Similarly, the third ablation setting uses a single vector for all individuals rather than a different vector for each individual and this also causes a performance drop, which means the individual vectors have captured some semantics of their individuals. 

%the video-captioning baseline suffers from a disadvantage that is not penalized in the above results. This baseline requires two successive transformations, video to natural language, and then natural language to logical language. This makes it slower and more awkward to employ, as two separate processes need to be run, and it also means there are two stages at which the system can produce errors. However, because the second stage, the transformation from natural language to logical language, is performed by the same system that was used to create the dataset, any errors that occur in this stage will not affect the baseline's results. All such errors would also have appeared in the creation of the dataset itself. Therefore, whenever the video-captioning network predicts the correct natural language caption, the baseline will automatically predict the `correct' logical annotation, i.e., the logical annotation present in the dataset. If such a two-stage system were employed in practice, it is quite possible that the video-captioning network predict the correct natural language caption, but the semantic parser make a mistake and so the final output, the logical annotation, be incorrect. 
%EG1 I wuouldn't call the second one a disadvantage, because our network has been trained on a dataset created by that parser, so "the perfect neural network" (i.e., the one that achieves 100% accuracy) would make the same mistake. I would talk about an advantage with respect to these metrics.

%We explore two different thresholding methods. The first, denoted fixed-thresh simply thresholds at 0.5 for all probability scores. The second, denoted variable-thresh, varies the threshold by leveraging a prior expectation of the number of atoms per video. The potential atoms are placed in inverse order of their probability scores, and then added to the annotation one at a time. The threshold increases with each added atom, reflecting the expectation that the correct number of atoms for a video is unlikely to be zero and unlikely to be very large. 


Secondly, the ablation studies show a greater drop in performance in the dataset MSR-VTT*, when ablating components of the decoder. This is also accounted for by the larger vocabulary size of MSR-VTT (and hence MSR-VTT*). Our decoder has a different MLP for each predicate, so a larger number of predicates means a larger number of MLPs, each of which can thus be more semantically specialized. Replacing all MLPs with a single MLP would then hurt the performance more. The same applies to the individual vectors.

%a number of words that do not describe the contents of the video directly, but rather a property of the video qua video. E.g., many captions in MSR-VTT and MSVD begin with ``In this video we see..'', ``This video depcits..'' or ``The narrator describes..'', which our data processing procedure would parse as ``see(we,...)'', ``depticts(video,...)'' and ``describes(narrator,...)''. Clearly, there is no pattern in the video pixels that indicates ``video'' or ``narrator'' or ``depicts''. The details of which words we exclude for this purpose can be found in the appendix. 

%Another point is that, current state of the art video-captioning networks, such as \cite{olivastri2019end}, that we used for comparison, are the result of years of research and optimization \cite{aafaq2019video}. They are trained on datasets that are manually constructed especially for video captioning, unlike our network which is trained only on an automatically generated dataset. Furthermore, video-captioning networks make use of language models in their decoders, which are themselves highly optimized and trained on large bodies of text. Given these advantages, it is encouraging that our network performs at a comparable level. 

Note that, as discussed in Section \ref{subsec:comp-with-baseline}, the video-captioning baseline suffers from a disadvantage that is not reflected in these results. If tested on a human-annotated dataset of logical annotations, it would be expected to perform worse, whereas our model would not. 

Tables \ref{tab:MSVD*-results} and \ref{tab:MSRVTT*-results} show that all models predict mostly negatives and metrics are dominated by true negatives (despite reweighting, as described in Section \ref{sec-method}). F1-score is a suitable single metric on which to compare results, as it harshly penalizes low positive accuracy, but also takes account of negative accuracy. Accuracy and F1-score are harsh metrics, as they pertain to whole atoms. An annotation could achieve 0 accuracy if it contained correct individuals, and correct predicates, but related them in the wrong way, e.g., $fold(paper, person)$ or $carry(person,paper)$ in Figure~\ref{fig:msrvtt-ex}. Despite this,  comparisons with the previous work by \cite{Vasile} and with the video-captioning baseline clearly demonstrate that our system has learned to extract some semantics from the input video. 

\begin{figure}
    \begin{multicols}{2}
    \includegraphics[width=0.5\textwidth]{imgs/MSVD_1955.png} \\
    
    \textbf{MSVD ground truth:} \\ 
    \text{A man is eating a banana.} \vspace{3pt}\\
    \textbf{MSVD* ground truth:} \\ 
    \textit{$eat(man,banana)$} \vspace{3pt}\\
    \textbf{Predicted individuals:} \\ 
    \text{$man$} \vspace{3pt} \\
    \textbf{Predicted atoms:}\\ 
    \text{$stand(man)$, $sit(man)$} \vspace{3pt} \\
    \textbf{Subset of inferences:} \\ 
    \text{$standing(person)$, $standing(male)$} \vspace{3pt} \\
    \textbf{Predicted caption from \cite{olivastri2019end}:}\\ 
    \text{a man is talking on the phone} \vspace{3pt} \\
    \textbf{Parsed caption (baseline):} \\ 
    \text{$talk(man)$}
    \end{multicols}
    \vspace{-2em}
    \caption{%
        The first frame from a video in the MSVD* test set, with the ground truth caption, the caption produced by \cite{olivastri2019end}, the logical annotation produced by our system and some further inferences that can be made on top of this logical annotation. Note that the class $banana$ was excluded as described in Section~\ref{sec-dataset}. Compared with a video captioning system, our output can be used to infer additional information about the video, such as the fact that it contains a male. 
    }
    \label{fig:msvd-ex}
\end{figure}

@article{hohenecker2019rrn,
  author    = {Patrick Hohenecker and
               Thomas Lukasiewicz},
  title     = {Ontology Reasoning with Deep Neural Networks},
  journal   = {arXiv preprint arXiv:1808.07980},
  year      = {2018},
  archivePrefix = {arXiv},
  eprint    = {1808.07980},
  timestamp = {Sun, 02 Sep 2018 15:01:57 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1808-07980},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}%journal   = {CoRR},journal={arXiv preprint arXiv:
  %volume    = {abs/1808.07980},url       = {http://arxiv.org/abs/1808.07980},
 
 Similarly, we can infer $drives(man,vehicle)$ from $drive(man,car)$ in Fig.~\ref{fig:msrvtt-ex2}. The relation $fold$ is a subclass of the relation $change$ in WordNet, so from the predicted fact $fold(person,paper)$, we can also infer the fact  $change(person,paper)$ in Fig.~\ref{fig:msrvtt-ex}. The natural language annotation, while semantically very similar to the ground truth natural language caption, is unable to leverage these inferences, and so is unable to indicate that the video depicts a person changing something (by folding it). 
 
 \footnotetext{This constitutes a slight error in the semantic parser, \textit{fold}(\textit{person, paper}) would be more accurate. See Section \ref{subsec:comp-with-baseline} for further discussion.} 
 
 
 
propose an approach to extract structured information about a video, which is achieved by modelling what happens in the video using a logical description.
Such logical annotations can then be used in logic-based automated processing, which we exemplify by making inferences in order to obtain a more complete description of the video.
We use the term {\sl ontology} to refer to a knowledge base of inference rules (e.g.,  $\forall x~man(x)) \Rightarrow mortal(x)$). Our vocabulary of {\sl individuals} is then the set of all classes that appear in the ontology. Intuitively, they refer to the objects that can be present in the video (e.g., $man$).  It is also easier to quantify the correctness of logical annotations. They can be measured using typical metrics such as accuracy and F1-score. The agreement between a ground truth and predicted natural language sentence, on the other hand, can only be quantified using specially designed metrics (e.g., BLEU \cite{papineni2002bleu}, METEOR \cite{banerjee2005meteor}, and LEPOR \cite{han2012lepor}). Recognizing the imperfection of each of these, results for natural language annotation models typically report scores on multiple metrics and are consequently difficult to interpret. \todo{This discussion moved into the shortcomings discussion}

The input to our model is a video and the output is a logical annotation built by listing all the {\sl facts} (which are of the form $white(paper)$) that hold true of the video. As no dataset for logical description extraction is currently available, we created our own, 
denoted MSVD* and MSR-VTT*, starting from two popular video captioning datasets: MSVD  \cite{chen2011collecting} and MSR-VTT \cite{xu2016msr},
respectively. We parsed the captions using a simple rule-based semantic parser, based on the Stanford~parser \cite{qi2018universal}, to obtain a logical description of each video. 


The neural architecture that we use is composed of a video encoder, followed by a decoder that first predicts the individuals that are present, and then predicts the relations that hold between them. The main advantage of this approach over annotating in natural language is that it enables the application of automated logic-based processing. For example, additional facts can be automatically inferred in order to  augment the information in the video annotation. Furthermore, it~is easier to assess performance: we can use accuracy and F1-score, rather than the complex, bespoke metrics used for comparing natural language sentences. Evaluating the performance on two popular video annotation datasets, MSVD and MSR-VTT, we achieve comparable results to a baseline of a video-captioning network followed by a semantic parser, and we significantly outperform the one existing work that aims to logically annotate videos.

\todo{remove this entire paragraph}
The processing of temporal visual information is a key element of intelligence. It has a long history of study among psychologists and cognitive scientists \cite{geremek2013perception}, who appreciated its central role in human cognition. In contrast, the problem of computer video understanding was, at its inception in the 1960s, thought to be easily solvable \cite{margaret2008mind}. 
In the intervening years, it has emerged that, in keeping with the complexity of the human visual system, it is far from simple for a machine to understand a video. It requires interpreting low-level, unstructured pixel data, and representing this data in terms of high-level structures, such as objects, properties, relations, movement, and scenes. 
However, 
as shown by recent progress, deep learning
seems to provide the tools for solving this task. 

For example, if the word ``dance''
%'scrub' appear 7 times is MSVD
appeared in only 5 training examples, then we would, as described in Section~\ref{sec-method}, create a corresponding MLP, $MLP_{dance}$ and train it only on these examples. It would not be possible for $MLP_{dance}$ to learn generalizable semantic properties of $dance$ using so few examples. 

\iffalse
\begin{enumerate}
    \item motivated by important... (i'd directly start with this)
    \item Videos are normally annotated with natural language (cite some examples)
    \item this comes with many shortcomings: (i) it is not possible to perform reasoning on the annotations, (ii) natural language is very noisy and models have to learn its structures, (iii) natural language metrics are often not as intepretable as more standard metrics like accuracy or f1-score. (analyse each of the above shortcomings here, there is already a discussion about (i), add discussion for (ii) and (iii)) <- you have done this in the "Further discussion" section, I think it's worth removing it and have it moved entirely to the introduction by discussing the above points (+translation)
    \item To solve the above shortcomings, in this paper we propose to annotate videos with logical annotations. 
    \item since no dataset exists for such task, we propose a methodology to automatically create logically annotated videos. (give some details on the methodology)
    \item We then take a first step in the solution of the above task by proposing a neural network that is able to produce logical annotations for videos. (give some details on the model) + example 1
    \item we test our neural network on MSVD* and MSR-VTT*, two datasets obtained from MSVD and MSR-VTT using our methodology.  (+details, e.g., why these datasets?)
    \item say which metrics are used and with which results.
    \item structure of the paper
\end{enumerate}
\fi


\iffalse
\begin{enumerate}
    \item Videos are normally annotated with natural language \item this comes with many shortcomings: (i) it is not possible to perform reasoning on the annotations, (ii) natural language is very noisy and models have to learn its structures, (iii) natural language metrics are often not as intepretable as more standard metrics like accuracy or f1-score. 
    \item To solve the above shortcomings, in this paper we propose to annotate videos with logical annotations. 
    \item since no dataset exists for such task, we propose a methodology to automatically create logically annotated videos. 
    \item We then take a first step in the solution of the above task by proposing a neural network that is able to produce logical annotations for videos. 
    \item we test our neural network on MSVD* and MSR-VTT*, two datasets obtained from MSVD and MSR-VTT using our methodology.
\end{enumerate}
\fi

